Deformed SPDE models with an application to spatial modeling of significant wave height

A non-stationary Gaussian random field model is developed based on a combination of the stochastic partial differential equation (SPDE) approach and the classical deformation method. With the deformation method, a stationary field is defined on a domain which is deformed so that the field becomes non-stationary. We show that if the stationary field is a Mat'ern field defined as a solution to a fractional SPDE, the resulting non-stationary model can be represented as the solution to another fractional SPDE on the deformed domain. By defining the model in this way, the computational advantages of the SPDE approach can be combined with the deformation method's more intuitive parameterisation of non-stationarity. In particular it allows for independent control over the non-stationary practical correlation range and the variance, which has not been possible with previously proposed non-stationary SPDE models. The model is tested on spatial data of significant wave height, a characteristic of ocean surface conditions which is important when estimating the wear and risks associated with a planned journey of a ship. The model parameters are estimated to data from the north Atlantic using a maximum likelihood approach. The fitted model is used to compute wave height exceedance probabilities and the distribution of accumulated fatigue damage for ships traveling a popular shipping route. The model results agree well with the data, indicating that the model could be used for route optimization in naval logistics.

==> application.tex <==

\section{Results}
\label{sec:application}


\input{results}


==> exceedance.tex <==

\section{Exceedance probability and extreme loads on ships}
\label{sec:exceedance}
For the application to significant wave heights, one is sometimes interested in calculating probabilities of exceeding a given threshold value along a shipping route. 
For instance, extreme sea conditions characterized by very large significant wave heights can lead to breakage of the hull instantaneously or over a very short time span. Therefore, it is important to have control of the risks of encountering such extreme sea states.

This corresponds mathematically to the probability of the random field exceeding the threshold on a given curve in $\gspace$.
The model proposed in Section~\ref{sec:model} is strictly spatial, therefore any realization of the model is assumed to persist unchanged over time. However, we start by formulating results for more general spatio-temporal models that are not necessarily Mat\'ern in $\dspace$ nor purely spatial. Thus, let $X(\psp,t)$ denote a spatio-temporal Gaussian random field  with mean value function $\mu(\psp,t)$  and standard deviation function $\std(\psp,t)$.
%
Consider a curve $\gamma(t) = (\psp(t), t)^T$, where $\psp \in \gspace$ and $t \in [0,T]$, and define $X_\gamma(t) = X(\psp(t),t)$ as the random field evaluated on the curve $\gamma$, with mean $\mu_\gamma(t)$ and standard deviation $\sigma_\gamma(t)$. 
Using Rice's method of moments \citep{lit:piterbarg}, we can derive an upper bound for the exceedance probability on the curve. Specifically, the following proposition gives a bound for the probability of $X$ exceeding a threshold $u$ along the curve.


\begin{prop}
\label{thm:exceedanceProb} 
Assume that $X(\psp,t)$ is differentiable in mean square sense and that both $\mu(\psp,t)$ and $\std(\psp,t)$ are differentiable with continuous partial derivatives. Further assume that the curve, $\gamma$, is differentiable with continuous partial derivatives, then
\begin{align}
&\prob{ \max_{t\in[0,T]} X_\gamma(t)>u } \le 
\int_{0}^T \std_{\dot{W}}(t) \phi\left( \frac{a(t)}{\std_{\dot{W}}(t)} \right) \phi\left(\frac{u-\mu_\gamma(t)}{\std_\gamma(t)}\right) dt\\
&\qquad+\frac{1}{2} \int_{0}^T a(t) \left[2\Phi \left(  \frac{a(t)}{\std_{\dot{W}}(t)} \right) -1\right] \phi\left(\frac{u-\mu_\gamma(t)}{\std_\gamma(t)}\right) dt
+
\Phi\left( \frac{\mu_\gamma(0)-u}{\std_\gamma(0)} \right)
.
\end{align}
Here, $\phi$ and $\Phi$ denotes the pdf and cdf of the standard normal distribution, 
$a(t) := \frac{u-\mu_\gamma(t)}{\std_\gamma(t)^2}\dot{\std}_\gamma(t) + \frac1{\std_\gamma(t)}\dot{\mu}_\gamma(t)$, 
and $\std_{\dot{W}}(t)$ is the standard deviation of the mean square derivative of $W(t) := \frac{X_\gamma(t)-\mu_\gamma(t)}{\std_\gamma(t)}$. 
\end{prop}
The proof of the proposition can be found in Appendix \ref{sec:proofs}. The upper bound is a good approximation of the actual exceedance probability for large values of $u$, which is our main concern when modeling wave heights.
%
It is worth noticing that the only spatial dependency in this formula is in the marginal variance of the derivative process $\dot{W}(t)$, i.e., $\std_{\dot{W}}(t)$. 
We will now show how this variance can be computed when $X(\psp,t)$ is defined using a spatial deformation. 
%connect this variance with the spatio-temporal random field in $\dspace_{\text{st}}$, i.e. the deformed space for a spatio-temporal process. 

In Section~\ref{sec:model} we referred to $\dspace$ as the space where our spatial model would be stationary, isotropic, and for which the correlation was Mat\'ern. 
We now make a similar definition for a spatio-temporal process. Assume that $X$ is defined through the deformation approach using a function $F : \dspace_s \times \dspace_t \rightarrow \gspace_s \times \gspace_t$ such that the process on $\dspace_s \times \dspace_t$ is stationary, and that for a fixed $\tilde{t}\in \dspace_t$, $X(\tilde{\psp}, \tilde{t})$ is stationary and isotropic. 

Let $\tilde{W}(\tilde{\psp},\tilde{t}) = W(\warp^{-1}(\psp,t))$ and denote by  $\tilde{W}'_x, \tilde{W}'_y,$ and $\tilde{W}'_t$ its partial derivatives. Then $\std_{\dot{W}}(t)$ can be computed using the following proposition.
\begin{prop}\label{thm2}
Let $\sigma^2_{ij} = \Cov(\tilde{W}'_i(\tilde{\psp},\tilde{t}), \tilde{W}'_j(\tilde{\psp},\tilde{t}))$, for $i,j \in \{x, y, t\}$. With $\Sigma = \{\std^2_{ij}\}_{i,j}$ as the corresponding covariance matrix we have
\begin{align}
\std^2_{\dot{W}}(t) &= \dot{\gamma}(t)^T J[\warp^{-1}](\gamma(t))  \Sigma J[\warp^{-1}]^{T}(\gamma(t)) \dot{\gamma}(t),
\end{align}
where $\dot{\gamma}(t) = [ \dot{x}(t), \dot{y}(t), 1 ]^T$ is the velocity of the curve at time $t$.
\end{prop}
The proof of the proposition can be found in Appendix \ref{sec:proofs}.
%
For the special case of a model which is constant over time, the elements in the third row and column of $\Sigma$ are zero. For the model in Section \ref{sec:model}, the Mat\'ern correlation in $\dspace$ yields $\sigma^2_{xx} = \sigma^2_{yy} = \frac{1  }{2(\nu-1)}$ and hence,    
\begin{align}
\std^2_{\dot{W}}(t) &= \frac{1}{2(\nu-1)} \dot{\psp}(t)^T J[\warp^{-1}]^{T}(\psp(t)) J[\warp^{-1}](\psp(t)) \dot{\psp}(t) \\
&= \frac{\damp^2(t)}{2(\nu-1)} \dot{\psp}(t)^T H^{-1}(\psp(t)) \dot{\psp}(t),
\end{align}
%where we let $\dot{\psp}(t) = [\dot{x}(t), \dot{y}(t)]$, i.e. disregarding the temporal dimension due to having a purely spatial model.

It is worth noticing that we need $\nu>1$ or equivalently $\alpha>1+d/2$ for the result to hold since the field is otherwise not mean-square differentiable.
%It is worth noting that the derivatives in mean square are not defined when $\nu \le 1$ since the Mat\'ern random field is then too rough to be almost surely differentiable.

==> modelproperties.tex <==
\section{Model properties}
\label{sec:modelProp}
We see that the deformation induces anisotropy of the solution to \eqref{eq:SPDEG} through the matrix $H(\psp)$. If we would have $\mathcal{D} = \mathbb{R}^d$,  the variance of the solution is
$$
\Var(X(\psp)) = \frac{\Gamma(\alpha-1)}{\Gamma(\alpha)(4\pi)^{d/2}\tau(\psp)^2}
$$
In this case, if one also has that the deformation is not varying spatially, the covariance of the solution to \eqref{eq:SPDEG} is stationary and given by
\begin{align*}
\Cov \left( \psp_1, \psp_2 \right) = \sigma^2 C_{\nu} \left( \damp \sqrt{(\psp_1 - \psp_2)^T H^{-1}(\psp_1 - \psp_2)  } \right), \quad \sigma^2 = \frac{\Gamma(\alpha-1)}{\Gamma(\alpha)(4\pi)^{d/2}}\frac{1}{\tau^2},
\end{align*}
where $C_{\nu}$ is the Mat\'ern correlation function in \eqref{eq:matern} with smoothness parameter $\nu = \alpha - d/2$  \citep{lit:khristenko}. Thus, the parameters $\kappa$, $\nu$ and $\sigma$ has the same interpretations as for the standard Mat\'ern covariance, and $H$ controls the anisotropy where eigenvectors of $H$ with larger eigenvalues corresponds to directions with longer correlation ranges. 

For the special case $\alpha=2$, \cite{lit:fuglstad, lit:fuglstad2} considered the related model 
$$
(\tilde{\kappa}^2 - \nabla \cdot \tilde{H} \nabla) u = \noise,
$$
where the functions $\tilde{H}(\psp)$ and $\tilde{\kappa}(\psp)$ could be chosen independently of each-other. Because of this, the marginal variance of the solution is affected by the choice of $\tilde{H}(\psp)$ and $\tilde{\kappa}(\psp)$.
In the stationary case, a direct consequence of comparing the covariance function of our model to the covariance function derived in~\citep{lit:fuglstad2} shows that the two models are equivalent (when using $\alpha = 2$ in our model). However, the important difference between the models (except for the general smoothness in our model) is that our parametrization allows for controlling the variance of the process independently of $\kappa$ and $H$. For the stationary case, this is not crucial, but when changing to non-stationary models it greatly simplifies estimation and parameter interpretations. 








